Blind Visible Watermark Removal with Morphological Dilation

Visible watermarks pose significant challenges for image restoration techniques, especially when the target background is unknown. Toward this end, we present MorphoMod, a novel method for automated visible watermark removal that operates in a blind setting -- without requiring target images. Unlike existing methods, MorphoMod effectively removes opaque and transparent watermarks while preserving semantic content, making it well-suited for real-world applications. Evaluations on benchmark datasets, including the Colored Large-scale Watermark Dataset (CLWD), LOGO-series, and the newly introduced Alpha1 datasets, demonstrate that MorphoMod achieves up to a 50.8% improvement in watermark removal effectiveness compared to state-of-the-art methods. Ablation studies highlight the impact of prompts used for inpainting, pre-removal filling strategies, and inpainting model performance on watermark removal. Additionally, a case study on steganographic disorientation reveals broader applications for watermark removal in disrupting high-level hidden messages. MorphoMod offers a robust, adaptable solution for watermark removal and opens avenues for further advancements in image restoration and adversarial manipulation.

==> figs/gettys.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/gettys.pdf}
    \caption{MorphoMod performance on images scraped from Getty Images.}
    \label{fig:gettys}
\end{figure*}

==> tabs/alpha_t.tex <==
\begin{table*}[t]
\caption{Semantic Preservation Performance Metrics}
\label{tab:alpha_expr_t}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccc|ccc}
\toprule
 \multirow{2}{*}{Model} &  \multicolumn{3}{c|}{Alpha1-S} & \multicolumn{3}{c}{Alpha1-L} \\ 
 & $RMSE_T (\downarrow)$ & $SSIM_T (\uparrow)$ & $LPIPS_T (\downarrow)$ & $RMSE_T (\downarrow)$ & $SSIM_T (\uparrow)$ & $LPIPS_T (\downarrow)$ \\
\midrule
SLBR  & 0.0067 & 0.9980 & 0.0036  & 0.0077 & 0.9984 & 0.0024  \\ 
SplitNet  & 0.0041 & 0.9993 & 0.0012  & 0.0049 & 0.9993 & 0.0012  \\ 
WDNet  & 0.0212 & 0.9845 & 0.0180  & 0.0255 & 0.9869 & 0.0134  \\ 
DENet-g  & 0.0056 & 0.9985 & 0.0026  & 0.0049 & 0.9990 & 0.0016  \\ 
DENet-h  & 0.0075 & 0.9985 & 0.0025  & 0.0176 & 0.9954 & 0.0070  \\ 
DENet-l  & 0.0043 & 0.9993 & 0.0012  & 0.0027 & 0.9997 & 0.0004  \\ 
$\text{morphomod}_0$  & 0.0108 & 0.9963 & 0.0041  & 0.0130 & 0.9958 & 0.0038  \\ 
$\text{morphomod}_1$  & 0.0125 & 0.9954 & 0.0045  & 0.0147 & 0.9948 & 0.0043  \\ 
$\text{morphomod}_3$ & 0.0157 & 0.9934 & 0.0060  & 0.0183 & 0.9928 & 0.0057  \\ 
$\text{morphomod}_5$  & 0.0191 & 0.9912 & 0.0078  & 0.0220 & 0.9906 & 0.0077  \\ 
$\text{morphomod}_10$  & 0.0290 & 0.9844 & 0.0150  & 0.0324 & 0.9844 & 0.0141  \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*} 

==> tabs/eval_combine.tex <==

\begin{table*}[t]
\caption{Inpainting experimental results of various experiments on the Alpha1-S and CLWD datasets for $\mathrm{RMSE}_W$ ($R_W$), $\mathrm{SSIM}_W$ ($S_W$), $\mathrm{LPIPS}_W$ ($LP_W$), BRISQUE (B), NIQE (N), and PIQE (P).  }
\label{tab:comb_expr}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{p{0.1cm}|c|cccccc|cccccc}
\toprule
 & \multirow{2}{*}{Var} &  \multicolumn{6}{c|}{Alpha1-S} & \multicolumn{6}{c}{CLWD} \\ 
 \cline{3-14}
&  & $R_W (\uparrow)$ & $S_W (\downarrow)$ & $LP_W (\uparrow)$ & B & N & P & $R_W (\uparrow)$ & $S_W (\downarrow)$ & $LP_W (\uparrow)$ & B $(\downarrow)$ & $(\downarrow)$ & P  $(\downarrow)$\\
 \midrule
\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{5.2}}}& P1 & 0.369 & 0.599 & 0.317 &  38.88 & 4.96 & 43.49 & 0.216 & 0.791 & 0.176 &  25.24 & 4.39 & 38.49 \\
 & P2 & 0.369 & 0.599 & 0.318 &  39.34 & 4.97 & 43.29 & 0.211 & 0.795 & 0.173 &  25.41 & 4.37 & 38.47 \\
 & P3 & 0.373 & 0.598 & 0.317 &  38.96 & 4.96 & 43.23 & 0.223 & 0.786 & 0.181 &  24.78 & 4.38 & 38.45 \\
 & P4 & 0.370 & 0.599 & 0.317 &  39.21 & 4.95 & 43.34 & 0.214 & 0.793 & 0.174 &  25.45 & 4.34 & 38.41 \\
 & P5 & 0.371 & 0.598 & 0.317 &  39.18 & 4.99 & 43.33 & 0.216 & 0.792 & 0.176 &  24.86 & 4.36 & 38.28 \\
 & P6 & 0.377 & 0.592 & 0.321 &  39.20 & 4.98 & 43.39 & 0.216 & 0.792 & 0.178 &  25.22 & 4.35 & 38.72 \\
 & P7 & 0.375 & 0.594 & 0.323 &  39.07 & 4.99 & 43.47 & 0.216 & 0.792 & 0.176 &  25.27 & 4.35 & 38.55 \\
 & P8 & 0.372 & 0.595 & 0.320 &  39.31 & 4.95 & 43.44 & 0.214 & 0.794 & 0.175 &  25.26 & 4.32 & 38.43 \\
 & P9 & 0.373 & 0.596 & 0.318 &  39.05 & 4.97 & 43.55 & 0.217 & 0.791 & 0.177 &  25.99 & 4.37 & 38.77 \\
 & P10 & 0.369 & 0.599 & 0.317 &  39.12 & 4.94 & 43.26 & 0.214 & 0.794 & 0.174 &  25.97 & 4.30 & 38.57 \\
 \midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{5.3}}} & Normal & 0.369 & 0.599 & 0.317 &  39.82 & 4.95 & 44.08 & 0.214 & 0.794 & 0.174 &  25.97 & 4.30 & 38.57 \\
&  Background & 0.369 & 0.600 & 0.316 &  39.84 & 4.94 & 44.13 & 0.213 & 0.795 & 0.174 &  24.92 & 4.25 & 37.22 \\
&  Black & 0.370 & 0.600 & 0.316 &  39.84 & 4.94 & 44.10 & 0.213 & 0.795 & 0.175 &  25.04 & 4.26 & 37.36 \\
&  Gray & 0.370 & 0.599 & 0.316 &  39.84 & 4.93 & 44.14 & 0.213 & 0.794 & 0.174 &  24.95 & 4.28 & 37.36 \\
&  White & 0.371 & 0.598 & 0.316 &  39.83 & 4.93 & 44.12 & 0.213 & 0.794 & 0.174 &  24.82 & 4.27 & 37.28 \\
 \midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{5.4}}} & SD2 &  0.369 & 0.599 & 0.317 &  39.12 & 4.94 & 43.26 & 0.214 & 0.794 & 0.174 &  25.97 & 4.30 & 38.57 \\
&  SDXL & 0.334 & 0.625 & 0.299 & 39.63 & 4.91 & 44.06 & 0.198 & 0.800 & 0.169 & 24.49 & 4.36 & 37.91 \\
&  LaMa & 0.350 & 0.594 & 0.247 & 39.59 & 4.92 & 43.37 & 0.167 & 0.837 & 0.111 & 24.18 & 4.35 & 36.97 \\
 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*} 


==> tabs/eval_models.tex <==

\begin{table*}[t]
\caption{Inpainting experimental results of various experiments on the Alpha1-S and CLWD datasets for $RMSE_W$ ($R_W$), $SSIM_W$ ($S_W$), $LPIPS_W$ ($LP_W$), BRISQUE (B), NIQE (N), and PIQE (P).  }
\label{tab:alpha_expr}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|cccccc|cccccc}
\toprule
 \multirow{2}{*}{Model} &  \multicolumn{6}{c|}{Alpha1-S} & \multicolumn{6}{c}{CLWD} \\ 
  & $R_W (\uparrow)$ & $S_W (\downarrow)$ & $LP_W (\uparrow)$ & B & N & P & $R_W (\uparrow)$ & $S_W (\downarrow)$ & $LP_W (\uparrow)$ & B $(\downarrow)$ & $(\downarrow)$ & P  $(\downarrow)$\\
 \midrule
 SD2 &  \\
 SDXL & 0.334 & 0.625 & 0.299 & 39.63 & 4.91 & 44.06 & 0.198 & 0.800 & 0.169 & 24.49 & 4.36 & 37.91 \\
 LaMa & - & -& - & 39.59 & 4.92 & 43.37 & - & - & - & 24.18 & 4.35 & 36.97 \\
 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*} 

